Scalable Analytics over Distributed Time-series Graphs using GoFFish

Graphs are a key form of Big Data, and performing scalable analytics over them is invaluable to many domains. As our ability to collect data grows, there is an emerging class of inter-connected data which accumulates or varies over time, and on which novel analytics - both over the network structure and across the time-variant attribute values - is necessary. We introduce the notion of time-series graph analytics and propose Gopher, a scalable programming abstraction to develop algorithms and analytics on such datasets. Our abstraction leverages a sub-graph centric programming model and extends it to the temporal dimension using an iterative BSP (Bulk Synchronous Parallel) approach. Gopher is co-designed with GoFS, a distributed storage specialized for time-series graphs, as part of the GoFFish distributed analytics platform. We examine storage optimizations for GoFS, design patterns in Gopher to leverage the distributed data layout, and evaluate the GoFFish platform using time-series graph data and applications on a commodity cluster.

==> arch.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Architecture \emph{(1 page)}}
\label{sec:arch}

bin packing subgraphs, size of slices are same. template loaded completely. instance slices loaded
on-demand, incrementally, slice is cached

benchmark to capture cache effect. Sequential vs random loading of instances.

implementation of gopher uses in-memory \emph{object} transfer for passing state between instances,
not serialized messages. However,
abstraction allows for additional optimizations such as temporal partitioning, persisting and delayed
execution, etc. 

\subsection{GoFS Optimizations for Design Patterns}

Engineering optjimzation using double numeric writable (binary serialization), multi core for even more parallel beyond
subgraphs, etc.



Rationale:
Ensure that we maximize pipelining and parallelism of GoFS/Gopher, and their interactions, while minimizing I/O latency (\# of unique files read) and maximizing I/O bandwidth (ensuring sustained disk reads, and across multiple machines).
Approach:
Do we iterate over all subgraphs (SubgraphScan), or are we interested in only some of them (SubgraphFilter)? Do we use some (Project) or all attributes (ProjectAll)? 
Do we need the template (Topology), a single instance (SingleInstance), or all instances within a contiguous period (RangeInstance)?
Do we have multiple supersteps? If so, do the supersteps operate on different subgraph, the same (single) or different instances?
 
Variables: \# of supersteps, topology only/single instance/all instances, some/all subgraphs

Gopher access pattern 1 (Single superstep, all subgaphs, topology/single instance only e.g. vertex count):

Gopher access pattern 2 (Single superstep, all subgaphs, topology/all instances e.g. edge weight average over time):

Gopher access pattern 3 (Multiple superstep, all subgaphs, topology/single instance e.g. pagerank):

Gopher access pattern 4 (Multiple superstep, all subgaphs, topology/single instance e.g. pagerank):

Gopher access pattern 1 (Single superstep):

The access pattern for Gopher is as follows:
In superstep \#1: Create a logical resultset that consists of all subgraphs <S1..Sm>for a particular period of time <T1..Tn>. Iterate and access the template and the first instance of each subgraph. Process the subgraphs for this instance and hold limited state information on each subgraph. Optionally, iterate over time and load the next subgraph instance for each subgraph. Update state for each subgraph.
In superstep \#2: Based on messages messages 

\subsection{Motivating co-design of Storage and Programming (Yogesh/Charith)}

We
also relax the time to be a duration rather than a fixed point to allow for a compact model as also
time skews.


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End: 

